Evading Curse of Dimensionality in Unconstrained Private GLMs via Private Gradient Descent

We revisit the well-studied problem of differentially private empirical risk minimization (ERM). We show that for unconstrained convex generalized linear models (GLMs), one can obtain an excess empirical risk of $\tilde O\left(\sqrt{{\texttt{rank}}}/\epsilon n\right)$, where ${\texttt{rank}}$ is the rank of the feature matrix in the GLM problem, $n$ is the number of data samples, and $\epsilon$ is the privacy parameter. This bound is attained via differentially private gradient descent (DP-GD). Furthermore, via the first lower bound for unconstrained private ERM, we show that our upper bound is tight. In sharp contrast to the constrained ERM setting, there is no dependence on the dimensionality of the ambient model space ($p$). (Notice that ${\texttt{rank}}\leq \min\{n, p\}$.) Besides, we obtain an analogous excess population risk bound which depends on ${\texttt{rank}}$ instead of $p$. For the smooth non-convex GLM setting (i.e., where the objective function is non-convex but preserves the GLM structure), we further show that DP-GD attains a dimension-independent convergence of $\tilde O\left(\sqrt{{\texttt{rank}}}/\epsilon n\right)$ to a first-order-stationary-point of the underlying objective. Finally, we show that for convex GLMs, a variant of DP-GD commonly used in practice (which involves clipping the individual gradients) also exhibits the same dimension-independent convergence to the minimum of a well-defined objective. To that end, we provide a structural lemma that characterizes the effect of clipping on the optimization profile of DP-GD.

==> appBackground_aistats.tex <==
\section{More Background on Convex Learning}
\label{sec:ermglm}

\begin{defn}[Seminorm]
Given a vector space $V$ over a field $F$ of the real numbers $\boldR$, a seminorm on $V$ is a nonnegative-valued function $\rho: V\to\boldR$ with the following properties. For all $a\in F$, and $\boldu,\boldv\in V$: 
\begin{enumerate}
    \item {\bf Triangle inequality}: $\rho(\boldu+\boldv)\leq \rho(\boldu)+\rho(\boldv)$.\vspace{-0.2cm}
    \item {\bf Absolute scalability}: $\rho(a\cdot\boldu)=|a|\cdot\rho(\boldu)$.
\end{enumerate}
\label{def:seminorm}
\end{defn}

\mypar{Lipschitzness, Convexity, and Smoothness}
We additionally require the following definitions to state our results. These properties usually govern the rate of convergence of an algorithm for optimizing ERMs. 

\begin{defn}[$\ell_2$-Lipschitz continuity]
A function $f:\calC\to\boldR$ is $L$-Lipschitz w.r.t. the $\ell_2$-norm over a set $\calC\subseteq\boldR^p$ if the following holds:
$\forall \theta_1,\theta_2\in\calC, \left|f(\theta_1)-f(\theta_2)\right|\leq L \cdot\ltwo{\theta_1-\theta_2}$.
\label{def:lip}
\end{defn}

\begin{defn}[(Strong) convexity w.r.t. $\ell_2$-norm]
A function $f:\calC\to\boldR$ is $\Delta$-strongly convex w.r.t. the $\ell_2$-norm over a set $\calC\subseteq\boldR^p$ if $\forall \alpha\in(0,1),(\theta_1,\theta_2)\in \calC\times\calC$: 
{\small\begin{align*}
& f(\alpha\theta_1+(1-\alpha)\theta_2) \leq
\alpha f(\theta_1)+(1-\alpha)f(\theta_2)-\Delta\frac{\alpha(\alpha-1)}{2}\ltwo{\theta_1-\theta_2}^2. 
\end{align*}}
\noindent Function $f$ is simply convex if the above holds for $\Delta=0$.
\label{def:sc}
\end{defn}

\begin{defn}[Smoothness]
A function $f:\calC\to\boldR$ is $\beta$-smooth on $\calC\subseteq\boldR^p$ if for all $\theta_1\in \calC$ and for all $\theta_2\in\calC$, we have
{\small\begin{align*}
f(\theta_2) \leq f(\theta_1) + \ip{\nabla f(\theta_1)}{\theta_2-\theta_1} + \frac{\beta}{2} \|\theta_1-\theta_2\|_2^2.
\end{align*}}
\label{def:smooth}
\end{defn}




